AMD-Hummingbird: Towards an Efficient Text-to-Video Model

Text-to-Video (T2V) generation has attracted significant attention for its ability to synthesize realistic videos from textual descriptions. However, existing models struggle to balance computational efficiency and high visual quality, particularly on resource-limited devices, e.g.,iGPUs and mobile phones. Most prior work prioritizes visual fidelity while overlooking the need for smaller, more efficient models suitable for real-world deployment. To address this challenge, we propose a lightweight T2V framework, termed Hummingbird, which prunes existing models and enhances visual quality through visual feedback learning. Our approach reduces the size of the U-Net from 1.4 billion to 0.7 billion parameters, significantly improving efficiency while preserving high-quality video generation. Additionally, we introduce a novel data processing pipeline that leverages Large Language Models (LLMs) and Video Quality Assessment (VQA) models to enhance the quality of both text prompts and video data. To support user-driven training and style customization, we publicly release the full training code, including data processing and model training. Extensive experiments show that our method achieves a 31X speedup compared to state-of-the-art models such as VideoCrafter2, while also attaining the highest overall score on VBench. Moreover, our method supports the generation of videos with up to 26 frames, addressing the limitations of existing U-Net-based methods in long video generation. Notably, the entire training process requires only four GPUs, yet delivers performance competitive with existing leading methods. Hummingbird presents a practical and efficient solution for T2V generation, combining high performance, scalability, and flexibility for real-world applications.

==> preliminary.tex <==
\section{PRELIMINARY: Video Diffusion Models}
% \yn{if the page space is not sufficient, move this PRELIMINARY to supp.}

Diffusion-based generative models have recently become prominent in image synthesis, defining a forward stochastic process that perturbs data samples \( x_0 \sim p_{\text{data}}(x) \) into progressively noisier representations, eventually yielding samples \( x_T \sim \mathcal{N}(0, I) \). This forward process \( q(x_t|x_0, t) \) comprises \( T \) discrete timesteps, each introducing incremental noise from \( x_0 \) to \( x_t \). %to the initial data \( x_0 \), parameterized to efficiently diffuse the structure of the data into pure Gaussian noise. 
The reverse or denoising process, defined as \( p_{\theta}(x_{t-1}|x_t, t) \), utilizes a neural network \( \epsilon_{\theta}(x_t, t) \) trained to approximate the noise added at each timestep, with the objective function: 
\begin{equation}    
    \min_{\theta} \mathbb{E}_{t, x \sim p_{\text{data}}, \epsilon \sim \mathcal{N}(0, I)} \| \epsilon - \epsilon_{\theta}(x_t, t) \|_2^2, 
\end{equation}
\noindent where \( \epsilon \) denotes the noise injected during diffusion, and \( \theta \) represents the learnable parameters of the network. 
In this paper, we build our method on top of a video Latent Diffusion Model (LDM)~\cite{ho2022imagen}, DynamiCrafter~\cite{xing2025dynamicrafter}. Specifically, given an input video \( x \in \mathbb{R}^{N \times 3 \times H \times W} \), we encode each frame to obtain a latent representation \( z = E(x) \) and perform the forward diffusion \( z_t = p(z_0, t) \) and the backward denoising process \( z_t = p_{\theta}(z_{t-1}, c, t) \) in this latent space, where \( c \) serves as a conditioning signal. As for the video frame interpolation setting in the work of DynamiCrafter~\cite{xing2025dynamicrafter}, the conditions include text description $c_{T}$ and both beginning frame $c_{I}^{1}$ and last frame $c_{I}^{N}$. The optimization objective for a video LDM is:
% {
% \baselineskip=3pt
\begin{equation}
     \min_{\theta} \mathbb{E}_{E(x), t, \epsilon \sim \mathcal{N}(0, I)} \| \epsilon - \epsilon_{\theta}(z_t;  t, \text{fps}, c_{I}^{1}, c_{I}^{N}, c_{T}) \|_2^2,
\label{eq:loss_ldm}
\end{equation}
% }
\noindent where \( t \) is the diffusion timestep, and \( \text{fps} \) denotes the FPS control introduced in~\cite{xing2025dynamicrafter}. The generated videos are then obtained through the decoder \( \hat{x} = D(z_0) \).
